Challenges and Opportunities in Improving Worst-Group Generalization in Presence of Spurious Features

Deep neural networks often exploit *spurious* features that are present in the majority of examples within a class during training. This leads to *poor worst-group test accuracy*, i.e., poor accuracy for minority groups that lack these spurious features. Despite the growing body of recent efforts to address spurious correlations (SC), several challenging settings remain unexplored.In this work, we propose studying methods to mitigate SC in settings with: 1) spurious features that are learned more slowly, 2) a larger number of classes, and 3) a larger number of groups. We introduce two new datasets, Animals and SUN, to facilitate this study and conduct a systematic benchmarking of 8 state-of-the-art (SOTA) methods across a total of 5 vision datasets, training over 5,000 models. Through this, we highlight how existing group inference methods struggle in the presence of spurious features that are learned later in training. Additionally, we demonstrate how all existing methods struggle in settings with more groups and/or classes. Finally, we show the importance of careful model selection (hyperparameter tuning) in extracting optimal performance, especially in the more challenging settings we introduced, and propose more cost-efficient strategies for model selection. Overall, through extensive and systematic experiments, this work uncovers a suite of new challenges and opportunities for improving worst-group generalization in the presence of spurious features. Our datasets, methods and scripts available at https://github.com/BigML-CS-UCLA/SpuCo.

==> benchmark.tex <==
\begin{table*}[!t]
\caption{Complete Results: Worst-group \& Average Group accuracy ($\%$) of training with SOTA algorithms. Early stopping is employed. * (taken from \cite{liu2021just}) \looseness=-1
}
\label{tab:all_tab}
\vspace{-3mm}
\begin{center}
\resizebox{1\textwidth}{!}{%
\begin{tabular}{|l|cc|cc|cc|cc|cc|cc|}
\toprule
 &\multicolumn{2}{c|}{\textsc{Waterbirds}} & \multicolumn{2}{c|}{\textsc{CelebA}} &  \multicolumn{2}{c|}{\textsc{UrbanCars}}&\multicolumn{2}{c|}{\textsc{SpuCoAnimals}} & \multicolumn{2}{c|}{\textsc{SpuCoSun} (Hard)}& \multicolumn{2}{c|}{\textsc{SpuCoSun} (Easy)}\\
 & WG & Average  & WG & Average   &  WG& Average&WG & Average    & WG & Average   & WG &Average   \\\midrule\midrule
 ERM& $80.1_{\pm0.7}$ & $97.8_{\pm 0.3}$  & $78.7_{\pm 2.1}$& $83.4_{\pm 3.5}$&  $56.8_{\pm 5.6}$ & $96.4_{\pm 0.5}$ & $39.0_{\pm 1.4}$ & $75.8_{\pm 1.8}$ & $29.3_{\pm 1.4}$& $96.0_{\pm 0.2}$& $21.9_{\pm 3.51}$& $96.7_{\pm 0.1}$\\\midrule\midrule
 EIIL & $83.5_{\pm 2.8}$ & $94.2_{\pm 1.3}$  & $78.9_{\pm 0.6}$ & $86.9_{\pm 2.0}$ &  $78.9_{\pm 2.8}$ & $90.2_{\pm 1.3}$ & $64.9_{\pm 3.5}$ & $77.3_{\pm 2.4}$ & $  65.9_{\pm 1.3}$&  $76.1_{\pm 3.1}$& $64.4_{\pm 3.2}$ &  $79.0_{\pm 4.2 }$\\
 JTT & $83.1_{\pm 3.5}$ & $90.6_{\pm 0.3}$  & $81.5_{\pm 1.7}$*& $88.1_{\pm 0.3}$*&  $68.3_{\pm 6.7}$ & $91.9_{\pm 4.4}$ &$57.4_{\pm 2.3}$&$83.6_{\pm 1.1}$& $55.8_{\pm 1.1}$&  $88.8_{\pm 0.6}$&  $63.5_{\pm 0.3}$ &  $85.1_{\pm 0.4}$\\
 \spare & $91.6_{\pm 0.8}$ & $96.2_{\pm 0.6}$  & $86.5_{\pm3.3}$ & $89.8_{\pm0.3}$ &  $80.5_{\pm 3.9}$ & $90.3_{2.5}$ & $61.6_{\pm 2.4}$& $76.5_{\pm 1.1}$ &  $62.2_{\pm 1.4}$&  $80.3_{\pm 1.8}$&  $66.3_{\pm 1.6}$&  $79.1_{\pm 1.4}$\\
 \midrule\midrule
 SSA & $85.1_{\pm 1.3}$ & $96.7_{\pm 1.6}$  & $89.4_{\pm 0.5}$& $91.2_{\pm 0.2}$&  $78.7_{\pm 2.6}$ & $93.4_{\pm 0.7}$ &$64.4_{\pm 3.1}$& $75.5_{\pm 1.4}$ & $68.7_{\pm 0.8}$& $83.9_{\pm 0.8}$& 
  $66.0_{\pm 0.6}$& $79.4_{\pm 4.9}$\\ 
 $\text{DFR}^{\text{Val}}_{\text{Tr}}$ & $90.6_{\pm 0.4}$ & $93.4_{\pm 0.2}$  & $89.1_{\pm 1.2}$ & $91.3_{\pm 0.1}$ &  $81.9_{\pm 1.2}$ & $92.5_{\pm 1.8}$ & $66.5_{\pm 1.8}$ & $80.0_{\pm 3.7}$  &$67.3_{\pm 1.6}$&$79.9_{\pm 2.6}$&$68.2_{\pm 0.7 }$&$80.1_{\pm 1.5}$\\
 \midrule\midrule
 GB & $88.1_{\pm 0.6}$ & $95.5_{\pm 0.4}$  & $88.6_{\pm 1.0}$& $91.1_{\pm 0.1}$&  $82.7_{\pm 2.0}$ & $92.8_{\pm 0.0}$ & $69.9_{\pm 0.1}$ & $79.1_{\pm 0.1}$ &  $69.9_{\pm 0.6}$& $79.1_{\pm 0.2}$& $64.4_{\pm 1.5}$&$78.1_{\pm 0.6}$\\
 GDRO & $85.7_{\pm 0.8}$ & $94.3_{\pm 1.0}$  & $89.4_{\pm 0.1}$& $91.4_{\pm 0.1}$&  $78.9_{\pm 2.6}$ & $92.7_{\pm 1.6}$ & $67.1_{\pm 0.2}$ &  $75.1_{\pm 0.1}$ &  $65.5_{\pm 2.3}$& $78.2_{\pm 0.8}$&$64.7_{\pm 1.8 }$&$77.4_{\pm 4.8}$\\
 PDE & $90.3_{\pm{0.3}}$& $92.4_{\pm{0.8}}$ & $91.0_{\pm{0.4}}$ & $92.0_{\pm{0.6}}$ & $84.3_{\pm 1.7}$ & $92.2_{\pm 2.0}$ & $70.1_{\pm 2.0}$ & $78.7_{\pm 1.0}$ &  $67.6_{\pm 0.8}$ & $77.7_{\pm 1.2}$& $66.0_{{\pm 2.7}}$&$77.4_{\pm 0.3}$\\ \bottomrule
\end{tabular}%}
}
\end{center}
\vspace{-5mm}
\end{table*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{Fig/main_results.pdf}
    \caption{Worst-group accuracy of 8 SOTA methods on 6 datasets with spurious correlations. 
    }
    \label{fig:all_bar}
\end{figure*}
\section{Benchmarking Worst-group Accuracy under Spurious Correlations}\label{sec:benchmark}


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{Fig/cvpr_new_figs/gap_avg_over_method_per_ds.png}
    \caption{\sj{Where shoould this go?}}
    \label{fig:enter-label}
\end{figure}


\begin{comment}
\begin{figure*}[t]
  \centering
  \begin{subfigure}{0.12\textwidth}
    \includegraphics[width=\linewidth]{Fig/min_in_maj/min_in_maj_Waterbirds.pdf}
  \end{subfigure}
  \begin{subfigure}{0.12\textwidth}
    \includegraphics[width=\linewidth]{Fig/min_in_maj/min_in_maj_CelebA.pdf}
  \end{subfigure}
  \begin{subfigure}{0.36\textwidth}
    \includegraphics[width=\linewidth]{Fig/min_in_maj/min_in_maj_UrbanCars.pdf}
  \end{subfigure}
  % \medskip % Add some space between the rows
  \begin{subfigure}{0.12\textwidth}
    \includegraphics[width=\linewidth]{Fig/min_in_maj/min_in_maj_SpuCoAnimals (CLIP).pdf}
  \end{subfigure}
  \begin{subfigure}{0.24\textwidth}
    \includegraphics[width=\linewidth]{Fig/min_in_maj/min_in_maj_SpuCoSUN.pdf}
  \end{subfigure}
  \caption{Number of minority examples inferred as the majority by the group inference methods.} \label{fig:min_in_maj}
\end{figure*}
\end{comment}



==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{} See code and data repository: \url{https://github.com/BigML-CS-UCLA/SpuCo} 
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> cost.tex <==
\subsection{Cost of Training and Model Selection}

% \begin{figure}
%     \centering
%     \begin{minipage}[t]{0.48\textwidth}
%     \includegraphics[width=\linewidth]{Fig/cost.pdf}
%     \caption{\sj{check if it fits?} Training time of different methods with bubble size representing total time and y-axis displaying robust training time. 
%     }
%     \label{fig:cost}
%     \end{minipage}%
%     \hfill
%     \begin{minipage}[t]{0.48\textwidth}
%     \includegraphics[width=\linewidth]{Fig/model_sel_cost.pdf}
%     \caption{Comparison of model selection costs for various algorithms, normalized to 1x ERM run. 
%     }
%     \label{fig:model_sel_cost}
%     \end{minipage}%
%     \vspace{-2mm}
% \end{figure}

\begin{figure}
    \includegraphics[width=\linewidth]{Fig/model_sel_cost.pdf}
    \caption{Comparison of model selection costs for various algorithms, normalized to 1x ERM run. 
    }
    \label{fig:model_sel_cost}
\end{figure}

% \textbf{Cost of Methods. } Fig. \ref{fig:cost} shows the wall-clock run time of %the group inference and robust training phases of 
% different methods relative to that of ERM. 
% % For group inference algorithms, the cost of the group inference and robust training is plotted separately. 
% % \footnote{EIIL and SSA use GDRO for Robust Training, hence they do not have a bar corresponding to Robust Training for them.}
% Among the group inference methods, \spare and EIIL are the most efficient, as they infer the groups early in training and do not increase the training cost subsequently. JTT is more expensive as it infers the groups later in training and considerably increases the training cost by upsampling the minority groups by a large factor.  
% Among the validation group-known methods, DFR is efficient but SSA is significantly costlier as it requires training a model to infer groups in a semi-supervised manner. 
% % \textbf{Group Inference} 
% % Group Inference typically involves training an ERM model for a few epochs and clustering the outputs of this model, thus is usually inexpensive, but SSA differs from this by training a model for spurious attribute prediction. SPARE and EIIL are equally efficient as they infer groups very early in training, JTT is slightly more expensive, with the optimal number of epochs to train the model for group inference often being larger. Finally, SSA is significantly costlier due to its distinct approach.
% % Robust Training trains the final model using the group information and requires at least as long than ERM, except for last-layer retraining methods. 
% Among the group-known methods, 
% PDE is slightly more efficient than ERM and GB. 
% %and JTT Train is far more costly than any other method. Last-layer retraining methods take a fraction of this cost but require access to a trained model to be applied. 


\textbf{Cost of Model Selection.} Worst-group accuracy is highly dependent on extensive model selection \cite{idrissi2022simple}. In fact, the cost of model selection is the most significant expense when using robust methods in practice. Fig. \ref{fig:model_sel_cost} shows the %number of hyperparameters for each method and the typical number of combinations explored for each method. 
time of model selection for different methods, relative to that of training the model with ERM.
All methods are tuned using the validation set worst-group accuracy. %for the resulting robust model. 
For group inference methods, this is extremely expensive as it requires training with the inferred groups for each hyperparameter combination and also tuning the robust training phase. 
% In Sec.  \ref{sec:model_sel:gi}, we consider how to reduce this cost. 

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{Fig/model_sel_cost.pdf}
%     \vspace{-3mm}
%     \caption{Cost of Model Selection \yy{DFR and CA numbers to be added}}
%     \label{fig:model_sel_cost}
%     \vspace{-3mm}
% \end{figure}
% \begin{table}
%     \centering
%     \begin{tabularx}{0.9\linewidth}{|c|c|c|}
%     \toprule
%          Method& hparams  & Grid Search Size \\ \midrule
%          ERM&  2& 9\\ \midrule
%          EIIL &  3& 18 * 9\\
%          JTT &  3& 36\\ 
%          \SPARE &  3& 18 * 9\\
%          SSA &  3& 9 * 9\\ \midrule 
%          GB &  2& 9\\
%          GDRO &  2& 9\\
%  PDE& 5&18\\
%  \bottomrule 
%     \end{tabularx}
%     \caption{Another bubble or something else?}
%     \label{tab:hparams}
% \end{table}

==> data.tex <==



%%%%%%%%%%%
% Extra animals details 
%%%%%%%%%%%%%%
%Compared to \water \cite{sagawa2020distributionally} that is artificially crea, \animal is sampled from real images, and has a more complex spurious features (background) with higher variation. To ensure this, we used the CLIP \cite{radford2021learning} zero-shot classification ability to extract ImageNet examples with particular backgrounds, using 
%the following template: \texttt{\{keyword\} background}. In classes \texttt{waterbirds} and \texttt{landbirds}, 
%for \textit{land} backgrounds we used keywords: \{\texttt{grass, forest, tree}\}, and for \textit{water} background we used keywords: \{\texttt{lake, river, sea}, \texttt{ocean}\}. 
%For classes \texttt{small dogs} and \texttt{big dogs}, 
%for \textit{indoor} background, we used keywords: \{\texttt{bed, couch and floor}\}. For \textit{outdoor} backgrounds we used keywords: \{\texttt{grass, park}, \texttt{road}\}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MOVE TO APPENDIX: 
% \textbf{Ensuring learnability of classes. } 
%%%%%%%%%%%%%%%%%%%%%%%%%
%To confirm the learnability of the classes in the absence of spurious features, we applied a fixed-sized mask to all images. The original image size is 256x256 pixels, and the spurious feature is scaled down to fit within a 112x112 pixel area. We train a {CLIP pre-trained ResNet-50} with ERM on the data using a 112x112 pixel mask to cover the area containing the spurious feature. \sj{emph: }\textit{In the absence of the spurious feature}, ERM achieves {76.8\%} accuracy with worst-group accuracy of 71.3\%, indicating that all the classes are indeed learnable.}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MOVE TO APPENDIX: 
% \textbf{Ensuring learnability of classes. } 
%%%%%%%%%%%%%%%%%%%%%%%%%
% As the bounding boxes for spurious features are not available, to ensure that the classes are learnable, we fine-tuned a pre-trained CLIP model with group-balancing (GB), which is an effective way to mitigate spurious correlations during training. This approach yields 70\% 
% %\ba{different in Table 2!} 
% worst group accuracy, confirming that the classes are learnable.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MORE DATASET DETAILS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SpuCoSun features four carefully curated classes, designed to reflect real-world environments and objects, ensuring the dataset’s realism and practicality. Each class combines specific background settings from SUN397 with corresponding spurious features from OpenImages V7. The classes are as follows:
% \begin{itemize}[label=--, left=0em, itemsep=0.5em]
%     \item \textbf{Recreational and Sports Environments:}
%     \begin{itemize}[label=$\circ$, left=1em, itemsep=0.5em]
%         \item Includes amusement parks, athletic fields, and indoor badminton courts.
%         \item Associated spurious features: sports equipment such as volleyballs, footballs, golf balls, and tennis balls.
%     \end{itemize}

%     \item \textbf{Residential and Living Spaces:}
%     \begin{itemize}[label=$\circ$, left=1em, itemsep=0.5em]
%         \item Focuses on residential and personal living spaces like attics, bathrooms, bedrooms, and dining rooms.
%         \item Associated spurious features: various fruits and vegetables like pumpkins, watermelons, tomatoes, broccoli, and bell peppers.
%     \end{itemize}

%     \item \textbf{Cultural and Educational Institutions:}
%     \begin{itemize}[label=$\circ$, left=1em, itemsep=0.5em]
%         \item Comprises locations like abbeys, amphitheaters, art galleries, and libraries.
%         \item Associated spurious features: different types of baked goods such as bread, cookies, muffins, bagels, and pretzels.
%     \end{itemize}

%     \item \textbf{Transportation and Infrastructure:}
%     \begin{itemize}[label=$\circ$, left=1em, itemsep=0.5em]
%         \item Covers transportation and infrastructure settings like airplane cabins, airport terminals, bridges, and train stations.
%         \item Associated spurious features: items related to containers and storage such as flowerpots, waste containers, bottles, beakers, and barrels.
%     \end{itemize}
% \end{itemize}

% Each class has 1 majority group (own spurious) and 3 minority groups (spurious of other 3 classes). The ratio of majority to minority is 67:1 in the training and validation set and 1:1 in the test set. The training set is approximately 32k images, the validation set is approximately 25\% of the size of the training set, and the test set consists of 250 images per group.



==> difficult_spurious.tex <==


% \subsection{Spurious Features of Different Learning Difficulty}\label{subsec: difficulty}

% \textbf{More difficult spurious features can still hurt WG Acc}

% \textbf{Group Inference is harder with more difficult SC}

% \textbf{Robust training can be more unpredictbale with more difficult SC}


% \textbf{now}
% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=\columnwidth]{Fig/difficult_spurious.png}
%     \caption{Performance gap between average accuracy and worst-group accuracy with varying levels of spurious feature difficulty. Green indicates low spurious difficulty, and red indicates high spurious difficulty. \sj{make like fig. 8} \yx{replot this with new numbers}}
%     \label{fig:difficult}
% \end{figure}


% Spurious correlations can have different levels of learning difficulty. In current literature, methods have rarely explored the differences in performance when presented with spurious correlations of different variances. In this section, we examine the impact of the variance in spurious features on learning in SpuCoSUN. In SpuCoSUN, the spurious features are objects from the OpenImages V7 dataset. Here, we control the number of subclasses selected for the minority groups. A larger number of subclasses corresponds to a higher spurious feature variance. The results are presented in \yx{Table \ref{tab:all_tab}'s last two columns and reorganized in} Figure \ref{fig:difficult}.
%where we illustrate the changes in the performance gap as the difficulty of the spurious features decreases.

% In SpuCoMNIST, the spurious features are colored background patchs. We keep the number of pixels in the colored background patch constant while allowing them to be selected from a broader range to increase the spurious variance. 

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=.152\textwidth]{Fig/hard_easy/Naive.eps}\includegraphics[width=.332\textwidth]{Fig/hard_easy/Group_Inference.eps}\includegraphics[width=.51\textwidth]{Fig/hard_easy/Group_Information.eps}
%     \caption{\yx{Easy spurious features reduce ERM's performance as expected. However, group inference methods' performance is negatively impacted by hard spurious features, with EIIL being an exception. In contrast, methods that have access to all or partial group information are relatively insensitive to difficulty of spurious features, with most of them experiencing a slight negative impact from easy spurious features. \ba{replace: show the gap.}}}
%     \label{fig:difficult}
% \end{figure}


% \yx{\textbf{ERM is negatively impacted by easy spurious features.} From the first plot in Figure \ref{fig:difficult}, we see that ERM's worst-group accuracy decreases by almost 10\% when spurious features become easier. This aligns with the intuition that the ease of spurious features makes the model more prone to relying on them. This also validates the construction of our datasets, indicating that the differentiation between hard and easy spurious features is meaningful.
% } 


% \begin{table}[!t]
%     \caption{\textbf{Group inference quality} of different methods on \textsc{SpuCoSun (Hard)}. Since group inference is essentially a binary classification by labeling data as majority or minority, we evaluate it based on accuracy, precision, and precision on minority groups. The last metric is particularly relevant as it measures how much of the data classified as minority are actually minority. \ba{replace Fig 3 with this, and drop here} }
%     \label{tab:groupinfperformance}
%     \centering
%         \begin{tabular}{|c|c|c|c|}
%         \hline
%         Method  & Inf. Acc. & Inf. Prec. & Inf. Prec. (minority) \\
%         \hline
%          EIIL & 97\% & 65\% & 52.2\% \\
%          JTT  & 95.2\% & 50.0\% & 39.2\% \\
%          SPARE & 66.8\% & 11.7\% & 9.6\% \\
%          \hline
%     \end{tabular}
%     % \begin{tabular}{|c|c|c|c|c|}
%     %     \hline
%     %     \multirow{2}{*}{Method}  & \multicolumn{2}{c|}{Accuracy} & \multicolumn{2}{c|}{Precision} \\
%     %     \cline{2-5}
%     %      & Hard & Easy & Hard & Easy \\
%     %      EIIL & 97\% & & 65\% & \\
%     %      JTT  \\
%     %      SPARE & 66\% & & 12\% & \\
%     % \end{tabular}
% \end{table}

% \yx{\textbf{Group inference methods are negatively impacted by hard spurious features, with the exception of EIIL.} 
%Another interesting and important observation concerns how different methods, particularly those without access to any group information (ERM, EIIL, JTT, and SPARE), behave under spurious features of varying difficulties. For this, we shall examine the last two columns of Table 2, comparing their performance on \textsc{SpuCoSun (Hard)} to that on \textsc{SpuCoSun (Easy)}.  
% Interestingly, we see that for group inference methods, two (JTT and SPARE) out of three show the opposite trend to ERM, performing worse on \textsc{SpuCoSun (Hard)}. Further analysis reveals that this observation is reasonable.  Remember that these methods rely on an ERM-trained model's early predictions/logits to identify data from different groups, and the underlying assumption is that the model learns the spurious features much faster than the core features. However, with hard spurious features, such an assumption can break down. The difficulty in spurious features makes their learning slower and less separable from the learning of core features, a phenomenon that has also been observed on toy datasets by \cite{qiu2024complexity}. However, we do see one exception, EIIL, which performs almost equally well on both \textsc{SpuCoSun (Hard)} and \textsc{SpuCoSun (Easy)}, suggesting that EIIL is less susceptible to hard spurious features. Table \ref{tab:groupinfperformance} confirms that EIIL's group inference is more accurate than others on \textsc{SpuCoSun (Hard)}. While it is challenging to determine the exact underlying reason, our best hypothesis is that this is because EIIL employs first-order information, unlike other methods. The expression of EIIL's objective in \cite{creager2021environment} suggests that the data is partitioned based on $(\text{logits} \times \text{gradient of loss w.r.t. logits})$ [TODO: can put a simple derivation in appendix], whereas JTT and SPARE primarily use zero-order information about logits. This additional information used by EIIL could explain its superior performance when groups are not well separated based solely on logits due to hard spurious features. We hope this can open up new insights for developing group inference methods that are more robust and able to handle situations with different levels of spurious feature difficulty. }


% Group Inference methods perform particularly poorly on datasets with more difficult spurious features. While they can match performance of methods with group labeled data (training or validation) on Waterbirds and CelebA, they are significantly worse on \textsc{SpuCoAnimals} and \textsc{SpuCoSun}. This demonstrates that the group inference is still unsolved in more challenging settings. 

%\ba{add minority in majority plots and use that to compare group inference part}




% \textbf{Group Inference Under-perform with Difficult Spurious Features.}\ba{what's the difference between this paragraph and 2 paragraphs ago?} Group Inference methods depend on accurately identifying and upsampling minority group samples to enhance performance. Consequently, while most GI methods exhibit a small gap between the worst-group accuracy and the average accuracy in cases with simple spurious features, where the spurious correlation is strongest, they face challenges when the spurious features become more varied and difficult to isolate. This suggests that the effectiveness of GI methods is closely tied to the strength of spurious correlations, potentially limiting their utility in more complex where the spurious correlations are more hidden.

% When the variance of the spurious feature shifts from high to low, fewer classes are selected for each minority group, resulting in a stronger spurious correlation. Although JTT and SSA exhibit poor performance in the worst-case group even with simpler spurious correlations, their accuracy declines further as the spurious correlation intensifies. EIIL, in particular, struggles with less varied spurious features, experiencing a 14\% drop in worst-group performance. This underscores the limited resilience of group inference methods when faced with challenging spurious features. 






% \textbf{Methods with Group Information Perform Consistently Across Various Spurious Difficulties.} Robust Training methods that incorporate group information substantially outperform all other algorithms. Among these methods, the performance gaps between average accuracy and worst-group accuracy are the smallest. While the performance gap is less pronounced in simpler datasets, such as Waterbird, as observed in Table \ref{tab:pretrain_crucial}, these methods also exhibit a more consistent performance gap across various levels of spurious variance compared to other approaches. This consistency indicates that group information becomes increasingly beneficial in the presence of stronger spurious correlations. However, when compared to the gaps observed in popular dataset benchmarks, where the performance gap is close to zero, there is still significant room for improvement. 

% \textbf{Limitations of Last Layer Retrain with Difficult Spurious Features.} Surprisingly, methods like DFR and LRMIX, while showing strong performances with less difficult spurious features and having a gap similar to methods with group information, such as GroupDRO, demonstrate a decline in performance as the variance of spurious features increases and the dataset exhibits weaker spurious correlation. Notably, LRMIX even shows a larger performance gap than ERM. This observation suggests that last-layer retrain methods are optimized for datasets with more uniform spurious features and depend on the strength of these correlations for making predictions. When confronted with more varied spurious features and less consistent spurious correlation, their performance may decrease significantly. 


% \textbf{Robust Training: more varied spurious features can still hurt WG Acc} For robust training methods like GB, GDRO, and PDE, trained on SpuCoMNIST, spurious features with lower variances lead to lower worst group accuracy, as the consistency of the spurious feature as the fixed colored patch makes the easier to rely on it during training. On the other hand, when trained on more realistic and difficult datasets like SpuCoSUN, surprisingly, the worst group accuracy increases as the spurious features become less varied and easier to learn. This is because for more varied spurious features, while the majority group has a more consistent patterned spurious feature, the minority group's spurious correlation also strengths, which can impact the overall reliability of the spurious correlation, thus leading to a drop of worst group accuracy.  

% \textbf{Group Inference is more challenging with stronger spurious correlation} For group inference method like JTT and SPARE, accurately identifying the minority group and correspondingly upsampling the correct samples is essential to the success of these methods. When trained on SpuCoMNIST, since the models have high prediction accuracy, they can correctly identify and upsample the minority group samples who are misclassified due to the strong spurious correlation. In a simple dataset like SpuCoMNIST, the weaker the spurious correlation is, the harder it is to identify the correct samples to upsample as the minority groups are more likely to be classified correctly. Consequently, contrary to Robust Training on SpuCoMNIST, the worst group accuracy decreases with more challenging spurious features. On the other hand, for more complex dataset like SpuCoSUN, in which the method cannot classify the samples well, stronger spurious correlation can lead to a decrease in worst group accuracy. 
% First 
% Finally, we examine the impact of the variance of spurious features on learning in SpuCoMNIST. The results are presented in Table 2. We observe that spurious features with a lower variance has a more drastic impact on the performance of the networks trained with ERM. In particular, low variance of the spurious features results in a worst-group accuracy that is a half of what ERM obtains under a high variance. %Hence, the network relies more on such spurious features and remains invariant to the core features of the majority groups. 
% At the same time, varying the variance of the spurious feature does not have a significant effect on the average accuracy of the network. For methods that utilize the group labels, like GDRO, GB, and PDE, a similar trend can be observed.However, for methods without any group labels, under low-to-high variance of the spurious feature, JTT suffers from very poor worst group accuracy. This is because JTT finds the minority group as misclassified examples at a given epoch. When learning the spurious feature is more difficult, the majority group is not learned reliably by any particular epoch and hence the minority group is more difficult to distinguish based on misclassification. For EIIL, a similar trend can be observed under low-to-medium variance of the spurious feature. SPARE which relies on the inference during the early training, on the other hand, are more robust to the variance change and achieves a comparable results to methods like GroupDRO and GB, which do have group labels. For methods that use group-labeled validation set like SSA, DFR and LRMIX, we also observe that lower variance of the spurious features can lead to lower performance, while DFR and LRMIX with last layer re-training are more robust to the variance change. 
% \begin{table}[h!]
% \centering
% \begin{footnotesize} % using smaller font size
% \setlength\tabcolsep{5pt} % reducing column padding
% \begin{tabular}{|l|cc|cc|cc|cc|}
% \hline
% \multicolumn{1}{|c|}{} & \multicolumn{4}{c|}{\textbf{SpuCoSUN}} & \multicolumn{4}{c|}{\textbf{SpuCoMNIST}} \\
% \cline{2-9}
% \textbf{Mtd} & \multicolumn{2}{c|}{\textbf{High}} & \multicolumn{2}{c|}{\textbf{Low}} & \multicolumn{2}{c|}{\textbf{High}} & \multicolumn{2}{c|}{\textbf{Low}} \\
% \hline
% & WG & Avg & WG & Avg & WG & Avg & WG & Avg \\ \hline
% ERM    & 20.2 & 46.1 & 20.2 & 47.9 & 44.3 & 99.8 & 44.6 & 99.8 \\
% GB     & 52.4 & 73.5 & 57.1 & 74.1 & 92.9 & 96.5 & 86.3 & 97.3 \\
% GDRO   & 53.6 & 70.8 & 59.5 & 79.9 & 91.4 & 96.9 & 84.3 & 98.3 \\
% JTT    & 22.6 & 43.5 & 19.0 & 47.1 & 75.1 & 97.7 & 82.7 & 97.4 \\
% SSA    & 21.4 & 49.8 & 25.0 & 48.2 & 87.8 & 94.1 & 83.7 & 98.9 \\
% DFR    & 36.9 & 73.7 & 48.8 & 72.5 & 92.2 & 97.1 & 90.7 & 97.1 \\
% LRMIX  & 34.5 & 83.1 & 48.8 & 74.8 & 92.2 & 96.5 & 91.2 & 95.7 \\
% SPARE  & 40.5 & 86.0 & 39.3 & 78.9 & 91.7 & 97.4 & 86.3 & 97.9 \\
% EIIL   & 46.4 & 75.5 & 32.1 & 70.5 & 43.7 & 99.7 & 53.5 & 99.6 \\
% PDE    & 56.0 & 71.7 & 58.3 & 72.5 & 88.4 & 91.4 & 85.1 & 94.1 \\
% \hline
% \end{tabular}
% \caption{Comparison of Methods on SpuCoSUN and SpuCoMNIST datasets }
% \label{table:merged_table}
% \end{footnotesize}
% \end{table}

% \begin{table}[h!]
% \centering
% % \begin{footnotesize} % using smaller font size
% % \setlength\tabcolsep{8pt} % reducing column padding
% \caption{Methods on SpuCoSUN with different spurious correlations }
% \begin{tabular}{|l|cc|cc|}
% \hline
% \textbf{Mtd} & \multicolumn{2}{c|}{\textbf{High}} & \multicolumn{2}{c|}{\textbf{Low}} \\
% \hline
% & WG & Avg & WG & Avg \\ \hline
% ERM    & $23.4_{\tiny\pm 3.0}$ & $61.6_{\tiny\pm 4.1}$ & $17.9_{\tiny\pm 1.9}$ & $58.1_{\tiny\pm 9.6}$ \\
% \hline
% JTT    & 22.6 & 43.5 & 19.0 & 47.1\\
% SSA    & $22.2_{\tiny\pm 3.0}$ & $71.8_{\tiny\pm 5.4}$ & $19.84_{\tiny\pm 3.9}$ & $46.6_{\tiny\pm 1.6}$\\
% SPARE  & 40.5 & 86.0 & 39.3 & 78.9\\
% EIIL   & 46.4 & 75.5 & 32.1 & 70.5\\
% \hline
% DFR    & 36.9 & 73.7 & 48.8 & 72.5\\
% LRMIX  & 34.5 & 83.1 & 48.8 & 74.8\\
% \hline
% GB     & $49.6_{\tiny\pm 3.9}$ & $72.8_{\tiny\pm 1.6}$ & $46.8_{\tiny\pm 7.3}$ & $71.3_{\tiny\pm 2.1}$\\
% GDRO   &  $52.0_{\tiny\pm 4.1}$ & $73.0_{\tiny\pm 1.5}$ & $54.4_{\tiny\pm 3.9}$ & $72.1_{\tiny\pm 1.7}$\\
% PDE    & $50.4_{\tiny\pm 4.4}$ & $71.92_{\tiny\pm 0.5}$ & 58.3 & 72.5\\
% \hline
% \end{tabular}
% \label{table:merged_table}
% % \end{footnotesize}
% \end{table}

% \sj{make figure, }
% \hy{ERM: low-> larger gap; wg down}
% \hy{all the other things opposite}
% \begin{table}[h!]
% \centering
% \begin{small}
% \begin{tabular}{|l|c|c|c|c|c|c|}
% \hline
% \textbf{Method} & \multicolumn{2}{c|}{\textbf{High}} & \multicolumn{2}{c|}{\textbf{Medium}} & \multicolumn{2}{c|}{\textbf{Low}} \\ 
% & WG & Avg & WG & Avg & WG & Avg \\ \hline
% ERM & 20.2 & 66.0 & 20.2 & 46.1 & 20.2 & 47.9 \\
% GB & 46.4 & 73.2 & 52.4 & 73.5 & 57.1 & 74.1 \\
% GDRO & 47.6 & 73.4 & 53.6 & 70.8 & 59.5 & 79.9 \\
% JTT & - & - & 22.6 & 43.5 & 19.0 & 47.1 \\
% SSA & 22.6 & 39.2 & 21.4 & 49.8 & 25.0 & 48.2 \\
% DFR & 38.1 & 67.9 & 36.9 & 73.7 & 48.8 & 72.5 \\
% LRMIX & 41.6 & 77.4 & 34.5 & 83.1 & 48.8 & 74.8 \\
% SPARE & 40.5 & 79.7 & 40.5 & 86.0 & 39.3 & 78.9 \\
% EIIL & 32.1 & 80.9 & 46.4 & 75.5 & 32.1 & 70.5 \\
% PDE & 54.8 & 78.4 & 56.0 & 71.7 & 58.3 & 72.5 \\
% \hline
% \end{tabular}
% % \caption{SpuCoSUN}
% \end{small}
% \label{table:your_table_label}
% \end{table}

% \begin{table}[h!]
% \centering
% \begin{small}
% \begin{tabular}{|l|c|c|c|c|c|c|}
% \hline
% \textbf{Model/Dataset} & \multicolumn{2}{c|}{\textbf{High}} & \multicolumn{2}{c|}{\textbf{Medium}} & \multicolumn{2}{c|}{\textbf{Low}} \\ 
% & Avg& WG& Avg& WG& Avg& WG\\ \hline
% ERM & 66.0 & 20.2 & 46.1 & 20.2 & 47.9 & 20.2 \\
% GB & 73.2 & 46.4 & 73.5 & 52.4 & 74.1 & 57.1 \\
% GDRO & 73.4 & 47.6 & 70.8 & 53.6 & 79.9 & 59.5 \\
% JTT & - & - & 43.5 & 22.6 & 47.1 & 19.0 \\
% SSA & 39.2 & 22.6 & 49.8 & 21.4 & 48.2 & 25.0 \\
% DFR & 67.9 & 38.1 & 73.7 & 36.9 & 72.5 & 48.8 \\
% LRMIX & 77.4 & 41.6 & 83.1 & 34.5 & 74.8 & 48.8 \\
% SPARE & 79.7 & 40.5 & 86.0 & 40.5 & 78.9 & 39.3 \\
% EIIL & 80.9 & 32.1 & 75.5 & 46.4 & 70.5 & 32.1 \\
% PDE & 78.4 & 54.8 & 71.7 & 56.0 & 72.5 & 58.3 \\
% \hline
% \end{tabular}
% \caption{SpuCoSUN}
% \end{small}
% \label{table:your_table_label}
% \end{table}

% \begin{table}[h]
% \centering
% \begin{small}
% \begin{tabular}{|l|ll|ll|ll|}
% \hline
% \textbf{Method} & \multicolumn{2}{c|}{\textbf{High}} & \multicolumn{2}{c|}{\textbf{Medium}} & \multicolumn{2}{c|}{\textbf{Low}} \\ 
% & WG & Avg & WG & Avg & WG & Avg \\ \hline
% ERM& 86.4    & 95.1      & 44.3    & 99.8      & 44.6    & 99.8      \\
% GB & 92.2    & 96.2      & 92.9    & 96.5      & 86.3    & 97.3      \\
% GDRO& 92.3    & 97.2      & 91.4    & 96.9      & 84.3    & 98.3      \\
% JTT& 32.5    & 96.2      & 75.1    & 97.7      & 82.7    & 97.4      \\
% SSA   & 97.1 & 92.2 & 94.1 & 87.8 & 83.7 & 98.9 \\
% DFR   & 92.0 & 98.1 & 92.2 & 97.1 & 90.7 & 97.1 \\
% LRMIX & 92.5 & 98.2 & 92.2 & 96.5 & 91.18 & 95.7 \\
% SPARE & 94.1 & 97.7 & 91.7 & 97.4 & 86.3 & 97.9 \\
% EIIL  & 91.7 & 96.0 & 43.7 & 99.7 & 53.48 & 99.58 \\
% PDE   & 91.9 & 94.4 & 88.4 & 91.4 & 85.1 & 94.1 \\
% \hline
% \end{tabular}
% \caption{SpuCo MNIST}
% \end{small}
% \label{table:your_table_label}
% \end{table}

% \sj{Make this a slope plot (\# 3 from examples)}
% \hy{Expectation: ERM: goes down -> YES; GB/GDRO/PDE: stable ->YES; GI:? LRT: goes up: More or LESS; }

% \hy{JTT-MNIST: up; SPARE-MNIST: slightly down; SSA-MNIST: slightly down; EIIL-MNIST: Significant down? (note) }

% \hy{JTT-SUN: down; SPARE-SUN: slightly down; SSA-SUN: slightly down; EIIL-SUN: significant down}

% \hy{JTT}
% \begin{table}[h]
% \centering
% \begin{small}
% \begin{tabular}{|l|ll|ll|ll|}
% \hline
% \textbf{Method} & \multicolumn{2}{c|}{\textbf{High}} & \multicolumn{2}{c|}{\textbf{Medium}} & \multicolumn{2}{c|}{\textbf{Low}} \\ 
% & Avg& WG& Avg& WG& Avg& WG\\ \hline
% ERM& 95.1    & 86.4      & 99.8    & 44.3      & 99.8    & 44.6      \\
% GB & 96.2    & 92.2      & 96.5    & 92.9      & 97.3    & 86.3      \\
% GDRO& 97.2    & 92.3      & 96.9    & 91.4      & 98.3    & 84.3      \\
% JTT& 96.2    & 32.5      & 97.7    & 75.1      & 97.4    & 82.7      \\
% SSA   & 92.2 & 97.1 & 87.8 & 94.1 & 98.9 & 83.7 \\
% DFR   & 98.1 & 92.0 & 97.1 & 92.2 & 97.1 & 90.7 \\
% LRMIX & 98.2 & 92.5 & 96.5 & 92.2 & 95.7 & 91.18 \\
% SPARE & 97.7 & 94.1 & 97.4 & 91.7 & 97.9 & 86.3 \\
% EIIL  & 96.0 & 91.7 & 99.7 & 43.7 & 99.58 & 53.48 \\
% PDE   & 94.4 & 91.9 & 91.4 & 88.4 & 94.1 & 85.1 \\
% \hline
% \end{tabular}
% \caption{SpuCo MNIST}
% \end{small}
% \label{table:your_table_label}
% \end{table}

==> group_inference.tex <==
\subsection{}

==> introduction.tex <==
\section{Introduction}

Machine learning models 
% achieve optimal performance when applied to data with the same distribution as their training data \cite{imagenet_cvpr09}. 
% However, they often 
perform poorly when there is a mismatch between their training and test distribution \cite{quinonero2008dataset}. 
\textit{Subpopulation shift} is a common type of distribution shift that characterizes the case when %all subpopulations exist in both training and test data, but 
the proportion of some subpopulations is different in the training and test data \cite{koh2021wilds}. 
% In such settings, models %may have high overall accuracy but 
% exhibit a poor \textit{worst-group} test accuracy 
% perform poorly 
% on subgroups that are small in training data, but may not necessarily be small in test data \cite{sagawa2020distributionally}.
A well-studied type of subpopulation shift occurs when data contains 
% spurious correlations
% A common cause of poor \textit{worst-group accuracy} under subpopulation shift is the existence of 
\textit{spurious correlations}---high correlations between domain-dependent features and labels in training data that do not hold in general \cite{sagawa2020distributionally}. 
% Under subpopulation shift, a common cause of poor worst-group accuracy is \textit{spurious correlations}, where models learn to associate the label to a simple and highly correlated feature that is irrelevant to the class. 
For example, if majority of images of a `swallow' appear on a `sky' background in training data, an image classifier may learn to associate the swallow category to the sky background instead of the bird. In this case, the model achieves a poor \textit{worst-group accuracy} on swallows that do not appear on sky background at test time. %Overparameterized models are particularly more prone to learning spurious correlations, as they 
% Spurious correlations cause models to predict the right labels for the wrong reasons and impede their generalization \cite{yang2023mitigating}. 

There has been a surge of recent efforts to develop techniques to learn classifiers that are robust to spurious correlations \cite{sagawa2020distributionally,liu2021just,nam2020learning,kirichenko2023last,yang2023identifying,deng2023robust}. 
%%%%%%%%%%
If majority and minority groups of examples with and without spurious feature are known, \textit{group-known} robust methods upweight or upsample the group to mitigate spurious correlations during training. Without the group information, \textit{group-inference} methods aim to infer the groups and then apply the group-known robust methods to alleviate spurious correlations. 
%%%%%%%%%%
However, there has been little work in evaluating SOTA algorithms to understand \textit{when} these methods can train robust classifiers, and how sensitive their performance is to the complexity\footnote{We characterize complexity of a feature by its learning speed. Complex features are learned later in training.} of the spurious feature. %in presence of spurious features of different learning difficulty. \ba{explan shift vs generalization vs wg}

In this work, we systematically investigate SOTA algorithms for improving worst-group test accuracy due to spurious correlations in \textit{vision} datasets. 
First, we introduce \textbf{3} more challenging image classification tasks with more complex spurious features. Then, we establish a comprehensive benchmark of \textbf{8} methods addressing poor worst-group accuracy due to spurious correlations and evaluate them on \textbf{6} datasets, including \textbf{3} existing vision benchmark datasets, and our \textbf{3} newly introduced datasets. %of different learning difficulties.
The modular implementation of our experimental framework facilitates the integration of new methods and datasets.
With over \textbf{5K} trained models, we demonstrate that, while the performance of SOTA methods is seemingly saturated on standard benchmark datasets, %with very strong spurious correlations, 
this important problem is indeed far from being solved in general.

% Specifically, [related/methods]

% Our work also evaluates current methods across different settings including the degree of spurious correlation, size of the validation set, pre-training algorithm and dataset, model architecture, and model selection strategies. 
% With the established framework and over \textbf{15K}  trained models, we reveal valuable observations for future research. 
% \sj{clarify that in our literature, you must see wg at train time and in the validation set.}
% \ba{explan shift vs generalization vs wg}



In summary, we make the following contributions:
\vspace{-2mm}
\begin{itemize}[leftmargin=20pt]
    \itemsep0em
    \item We introduce \textbf{3} new and more challenging vision datasets, with more complex spurious features. %that are significantly more challenging for existing methods.
    \item We develop a comprehensive benchmark for the problem of poor worst-group accuracy due to spurious correlations in vision datasets, evaluating \textbf{8} SOTA methods on \textit{6} datasets, including \textbf{3} existing benchmark datasets and our \textbf{3} newly introduced datasets.
    \item Based on over \textbf{5K} trained models, we find that: (1) group-known algorithms cannot effectively bridge the gap between worst-group and average accuracy, when the task is more challenging; (2) group-inference methods struggle to infer groups when spurious feature is more complex.
    % only improve worst-group accuracy under a limited range of spurious correlations and validation set size identified by our framework, but not others.\looseness=-1
    % \item \sj{no longer true?: We discover, perhaps surprisingly, that using architectures trained with CLIP ResNet-50 may be more susceptible to spurious correlations than pre-training with Supervised Learning on ImageNet.}
    \item We find a model selection criterion that can %be \textbf{100x} more efficient and nearly as effective.
    reduce substantial cost of model selection for group inference methods to 1\%. Besides, we show that with careful model selection, methods to tackle single spurious correlations can mitigate multiple spurious correlations.
\end{itemize}
% \vspace{-2mm}


\begin{comment}
\begin{itemize}
    \item Discuss the phenomenon of neural networks achieving high accuracy on i.i.d. test sets.
    \item However such networks may struggle in the presence of distribution shift, in particular achieve poor worst-group accuracy
    \item Distribution shift can refer to a wide-variety of sub-problems: SC, CI AI, AG, with each having different methods to address it
    \item Here we focus on poor worst-group accuracy due to SC i.e. poor accuracy on groups that are underrepresented in the training data due to the model relying on spurious correlations 
    \item However, while it may look like SC is relatively solved (cite Change is Hard), here we show that this is not true and illustrate concretely the several open problems that remain in the SC literature. \textbf{OR} While prior work like Change is Hard has studied SC, we find that many conclusions that hold for other kinds of distribution shift problem, do not hold for SC?
    \item We establish a detailed benchmark of SC consisting of xx SOTA algorithms that span different learning strategies and xx real-world datasets in vision and language(?) training over xxxx models to show the open problems that still remain in this field.
    \item List contributions?
\end{itemize}
\end{comment}

==> main_result_analysis.tex <==
\subsection{Analysis}
We study model performance over 6 different datasets, including three existing and our three new datasets. 

Fig. \ref{fig:all_bar} and Table \ref{tab:all_tab} show the results, where we make intriguing observations as follows. Hyperparameters to reproduce these results appear in Appendix \ref{appendix:hparams_main}.




% \textbf{Retraining Last Layer is Highly Effective.} 



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> multiple_spurious.tex <==
\textbf{Model Selection under Multiple Spurious Features} We further study model selection on \cars \cite{Li_2023_CVPR_Whac_A_Mole}, a dataset with two classes and two spurious features in each class--background (BG) and co-occurring object (CoObj). The dataset includes four groups: (1) common BG \& common CoObj, (2) common BG \& uncommon CoObj, (3) uncommon BG \& common CoObj, and (4) uncommon BG \& uncommon CoObj. Common BG \& common CoObj refer to the background and co-occurring object that is frequently associated with a particular class. %, and ``common CoObj" refers to the co-occurring object that is frequently associated with the same target class. 
The training set is highly imbalanced with respect to these spurious features: the majority of images (90.25\%) contain both common BG \& CoObj, while the remaining groups contain one or both uncommon features. When multiple spurious features exist, mitigating one can amplify reliance on others.\looseness=-1


% , and we found that using a small learning rate and large weight decay is most effective for handling multiple spurious features.}
% careful model selection can significantly improve performance on this dataset. \sj{improve with respect to original results? but we dropped comparison between our results and urban cars results from Table \ref{tab:multiple-compare}? should we add these bars to the figure? or somewhere else} 
% \ba{first say why this section/discussion matters}
% \textbf{Model selection with single spurious feature labels still helps.}  
% Our experiments demonstrate that model selection with single spurious feature labels still helps. \ba{in validation?}
We manipulated the validation set to include images where either one or both spurious features (BG and CoObj) appear. %Interestingly, %our analysis revealed
% \cref{tab:partial} shows no significant difference in the performance between the two variations, when careful model selection was employed. 
Remarkably, \cref{tab:partial} shows no significant difference in the performance (except SSA) between the two variations. This confirms, in contrast to \cite{Li_2023_CVPR_Whac_A_Mole}, that with careful model selection, methods designed for addressing one spurious correlation can indeed tackle multiple spurious correlations.
This finding is particularly significant as it suggests that effective model selection can substantially improve performance, even with partial group labels, which is a typical case in real-world data. \looseness=-1
% \ba{this paragraph is out of context here, say what is wg in this data, what are proportions, etc. give some context for this to make sense.}
% \ba{fix: we don't have spurious label, we have group label}

%It highlights that a well-thought-out model selection process is capable of handling incomplete or varied spurious feature scenarios, a common challenge in real-world data. 



% \begin{table}[h]
% \centering
% \begin{tabular}{|l|cc|cc|cc|}
% \hline
% \textbf{Model} & \multicolumn{2}{c|}{\textbf{BG only}} & \multicolumn{2}{c|}{\textbf{CoObj only}} & \multicolumn{2}{c|}{\textbf{Both}} \\ 
% & Wg & Ave & Wg & Ave & Wg & Ave \\ \hline
% ERM& 55.2 & 96.7 & 48.0 & 96.4 & 56.8 & 97.0 \\
% GB & 84.4 & 92.8 & 78.4 & 96.6 & 84.8 & 93.3 \\
% GDRO & 75.2 & 94.1 & 80.0 & 93.5 & 80.0 & 90.9 \\
% PDE & & & & & &  \\
% JTT & 70.4 & 92.4 & 57.6& 90.8& 76.0 & 91.8 \\
% SSA&         &           &         &           &         &           \\
% CNC&         &           &         &           &         &           \\
% DFR&         &           &         &           &         &           \\
% LRMIX&         &           &         &           &         &           \\
% LFF&         &           &         &           &         &           \\
% EIIL& 79.2 & 93.0  & 76.8 & 90.0 & 79.2 & 91.5 \\ 
% SPARE & 80.0 & 96.5 & 80.0 & 96.5 & 76.0 & 96.1 \\
% \hline
% \end{tabular}
% \caption{\yy{Will become a figure}}
% \label{tab:partial}
% \end{table}

\begin{figure}[!t]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Fig/multiple_spurious_val.pdf}}
\vspace{-1mm}
\caption{{Worst-group accuracy (\%) for different methods on the \cars dataset, with three labeling scenarios: background labels only (BG only), co-occurring object labels only (CoObj only), and labels of both spurious features (Both). The results indicate that model selection with single spurious feature labels (BG only or CoObj only) still helps, with no significant difference in performance (except SSA), compared to using labels of both spurious features.} 
}
\label{tab:partial}
\end{center}
\vspace{-8mm}
\end{figure}


% \begin{table}[h]
% \centering
% \begin{tabular}{|l|cc|cc|cc|}
% \hline
% \textbf{Model} & \multicolumn{2}{c|}{\textbf{BG only}} & \multicolumn{2}{c|}{\textbf{CoObj only}} & \multicolumn{2}{c|}{\textbf{Both}} \\ 
% & Ave & Wg & Ave & Wg & Ave & Wg \\ \hline
% ERM& 96.7 & 55.2 & 96.4 & 48.0 & 97.0 & 56.8 \\
% GB & 92.8 & 84.4 & 96.6 & 78.4 & 93.3 & 84.8 \\
% GDRO & 94.1 & 75.2 & 93.5 & 80.0 & 90.9 & 80.0 \\
% PDE & & & & & &  \\
% JTT & & & & & & \\
% SSA&         &           &         &           &         &           \\
% CNC&         &           &         &           &         &           \\
% DFR&         &           &         &           &         &           \\
% LRMIX&         &           &         &           &         &           \\
% LFF&         &           &         &           &         &           \\
% EIIL& 93.0 & 79.2  & 90.0 &  76.8 & 91.5  & 79.2 \\ 
% SPARE & 96.5 & 80.0 &  96.5 & 80.0  & 96.1 & 76.0 \\
% \hline
% \end{tabular}
% \caption{}
% \label{tab:partial}
% \end{table}




==> new_introduction.tex <==
\section{\sj{Intro}}

\sj{Sketch: 
\begin{enumerate}
    \item Introduce distribution shift, why it's important, and the types of DS (explain DG and SC), state we target SC in this paper 
    \item others are well-supported by challenging datasets, but not SC. many challenging settings have not yet been captured in existing datasets. we show three such dimensions for increasing the difficulty of SC datasets and cerate datasets to realize this. We then conduct a thorough benchmarking on these datasets (existing and new) to uncover what is still unsolved in SC. 
    \item Explain SC in detail (but already done before perhaps?). introduce groups and core v/s spruious feature. 
    \item More groups make the problem more difficult. More groups leads to larger gaps between wg and avg accuracy indicating poorer robustness to the spurious correlation. 
    \item More classes, also makes the problem more difficult in terms of sustaining average accuracy. different methods vary significantly on this, and this happens only when we add more clasess. This uncovers a new direction for future work to care about. 
    \item more diff spurious feature. group inference methodfs rely on easiness of spruious features. However, this leaves them vulnerable to slightly more complex spuripous features. These settings remain chalelnging for ERM, hence do require methods for spurious correaltions to be applied. but group inference mthods find them far more challenigng. 
    \item these are summarized in Fig. \ref{fig:intro_fig}
    \item Finally, in addition to benchmarking current methods in the aforementioned settings, we also investigate model selection on the more chalelning datasets. We show 1) model selection is extremely crucial 2) group inference model selection is extremely expensive \& can be made cheaper through direct group evaluation 3) model selection for multiple spurious features
\end{enumerate}
}

\begin{figure*}[ht]
    \centering
    \includegraphics[width=1\linewidth]{Fig/cvpr_new_figs/spuco_intro_fig_color2.pdf}
    \caption{Enter Caption \yy{We may want to make it clear what it means to have higher values on the y-axis for these 3 figures. We can also note where the existing benchmark datasets vs our datasets land in these 3 plots.}\yy{And we are the first to find these correlations, right? If so, we should highlight this? }}
    \label{fig:intro_fig}
\end{figure*}

Machine learning models typically perform reliably when training and test data share the same distribution. However, their performance often degrades significantly under distribution shift—when this assumption \yy{be more specific about which assumption} does not hold. In real-world scenarios, we constantly encounter distribution shifts. In domains such as medicine or autonomous driving, the failure of models to generalize under distribution shift can have serious real-world consequences. Therefore, robustness to distribution shift is one of the most critical open problems in machine learning. However, distribution shift is a broad issue. To address this \yy{to address the ds problem better? (instead of addressing that it is a broad issue)}, \cite{yang2023change} introduced a categorization of distribution shift types into: 1) Spurious Correlations, 2) Class Imbalance, 3) Domain (Attribute) Imbalance, and 4) Domain Generalization. \sj{1-2 line comparison between DG and SC}. In this work, we focus specifically on \textbf{spurious correlations}, a highly prevalent form of distribution shift. For example, \citeauthor{singla2022salientimagenetdiscoverspurious} demonstrates that models trained on ImageNet \yy{cite} \yy{for object classification?} often rely on spurious background features, which can reduce performance when objects appear in novel contexts.

While other types of distribution shift, such as domain generalization or imbalance, are well-supported by numerous datasets that pose challenging settings for current state-of-the-art (SOTA) algorithms \cite{zhang2023nico++, domainbed, koh2021wilds}, the same is not true for the spurious correlations problem. Datasets for studying spurious correlations are limited, and many challenging scenarios remain unaddressed, creating the false impression that the spurious correlations problem has been largely solved. In this paper, we introduce datasets that capture three distinct factors, each of which can make the spurious correlations problem more challenging for current methods. We then conduct a comprehensive benchmarking of SOTA methods on both existing and newly introduced datasets, highlighting several open problems in addressing spurious correlations.

\sj{some definition of group, spurious feature, core feature is needed now}. \yy{Maybe fig 2 will be helpful}

\sj{\textbf{more groups, more classes}}
One factor that influences the difficulty of addressing spurious correlations is the \textbf{number of groups} in the dataset. Figure \ref{fig:gap_vs_num_groups} illustrates how the gap between worst-group accuracy and average accuracy correlates with the number of groups in various datasets. \sj{explain why looking at gap?}. M\yy{any?} spurious correlation methods rely on hyperparameter tuning and use worst-group accuracy on the validation set as a metric. As the number of groups increases, this metric becomes less reliable, complicating model selection and making the task more challenging \yy{refer to section?}. In our work, we introduce three new datasets designed to address this issue by incorporating more groups than existing datasets. While UrbanCars is a recent dataset that also explores more groups by including multiple spurious features, we focus on an alternative approach: introducing more classes to create more groups. We show that this approach highlights its own unique challenges, such as significantly reduced average accuracy, when improvements in worst-group accuracy are achieved \yy{refer to section?}. 



\sj{\textbf{diff spurious}}
Another key factor is the difficulty of the spurious feature, defined by \citeauthor{yang2023identifying} as how early a feature is learned during training: easy features are learned early, while difficult features are learned later. \citeauthor{yang2023change} showed that ERM learns spurious features since they are easier than the true class feature. Methods that infer group membership from the data to remedy spurious correlations \yy{May need more context here to show what these methods are and why we care about them}, often rely on this observation i.e. the easiness of the spurious feature. Thus, while a more difficult spurious feature is less problematic for ERM i.e. worst-group accuracy is higher; for methods to infer group membership to remedy spurious correlations, the is more problematic i.e. worst group accuracy is lower. \yy{This paragraph needs to be further aligned with the bullet point}

To facilitate research in this area, we propose a new benchmark called \textbf{SpuCo}, specifically focused on spurious correlations in vision datasets. SpuCo includes two new datasets and incorporates a recent challenging dataset \yy{which one is the recent challenging dataset? Isn't it also new/what we want to propose? } to explore the impact of (1) more groups and (2) more difficult spurious features. Our contributions include:

\begin{itemize}[leftmargin=20pt]
    \item \textbf{Three new vision datasets}: a real-world dataset called \animals, with four classes, eight groups, and more difficult spurious features, and two synthetic datasets called \sun with four classes and 16 groups. The two versions of \sun (Easy Spurious and Hard Spurious) share the same core image features, but the Hard Spurious version includes more difficult-to-learn spurious features to facilitate controlled studies.
    \item \textbf{A comprehensive benchmark} evaluating eight SOTA methods across six datasets, including our new datasets and three existing benchmarks.
    \item \textbf{Extensive experimental analysis} involving over 5,000 trained models. Our findings show that: (1) group-known algorithms struggle to close the gap between worst-group and average accuracy as the problem becomes more complex, and (2) group-inference methods face challenges in inferring groups when spurious features are more difficult to learn.
    \item \textbf{A cost-effective model selection criterion} that reduces the expense of model selection for group inference methods to 1\%, demonstrating that with thoughtful model selection, methods designed for single spurious correlations can handle multiple spurious correlations.
\end{itemize}

In summary, our work shows that spurious correlations remain a significant and unsolved problem in machine learning. The insights from our study can inspire future research to develop more robust solutions to this critical challenge.



==> preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> pretraining.tex <==
% \subsection{Pre-training Weights \& Architecture}

% \yx{i think we no longer have results for this part after we changed the dataset right?}

% % \begin{figure}
% %     \centering
% %     \includegraphics[width=.23\textwidth]{Fig/pretrain/per_method.png}
% %     \includegraphics[width=.23\textwidth]{Fig/pretrain/per_dataset.png}
% %     \caption{Pretrain}
% %     \label{fig:pretrain}
% % \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=.23\textwidth]{Fig/pretrain/per_dataset.eps}
%     \includegraphics[width=.23\textwidth]{Fig/pretrain/per_method.eps}
%     \caption{Pretrain. We report the average worst-group accuracy over  methods per dataset, and over datasets per method. \sj{keep as is, maybe make prettier} \ba{see if we find any other model than CLIP}}
%     \label{fig:pretrain}
% \end{figure}

% % two suprising findings (1) clip-pretrained model performs the worst. (2) resnet18 is competitive with resnet 50 and even outperforms resnet50 in a few cases. 

% % \begin{itemize}
% %     \item Datasets: ImageNet, OpenAI CLIP dataset, (other pretrained we may find online)
% %     \item Algorithms: Supervised Learning, SimCLR on ImageNet (or some contrastive), CLIP
% %     \item Architecture: RN18 v/s RN50 v/s ViT
% % \end{itemize}

% % \begin{table*}[t]
% % \caption{\yx{todo: maybe remove the first column. change the heads}
% % \yx{Title:  Finetuning from Pretrained Weights is Crucial for Achieving Good Performance Across Methods on Waterbirds.}
% % Worst-group  and average accuracy ($\%$) of training with state-of-the-art algorithms on Waterbirds. CB, GB indicate balancing classes and groups, respectively. * indicates using data augmentation, and 
% % %Methods with (*) use data augmentation.
% % %\ba{fix the cost column, add group balancing with augmentation.}
% % $\diamond$ indicates that early stopping is not used. 
% % %This choice is made for ERM w/o augmentation to ensure consistency with the reported setting.  For ERM w/ augmentation, early stopping was not used in previous work \cite{kirichenko2022last} but used in our experiments.  
% % For all the other methods, we apply early stopping based on the worst-group validation accuracy.} 
% % \label{tab:pretrain_crucial}
% % \vspace{-3mm}
% % \begin{center}
% % \resizebox{0.9\textwidth}{!}{%
% % \begin{tabular}{|lcc|rr|rr|rr|}
% % \toprule
% %  & Group & Train & \multicolumn{2}{c|}{\bf Reported (pretrained)}  &\multicolumn{2}{c|}{\bf \spuco (pretrained)} &\multicolumn{2}{c|}{\bf \spuco (from-scratch)}  \\
% %  & Info & Cost & Worst-group & Average & Worst-group & Average & Worst-group & Average \\
% %  \midrule\midrule
% %  ERM$^\diamond$ & $\times$ & 1x & $60.0$ & $97.3$ & $65.7_{\pm 0.0}$ & $97.3_{\pm 0.0}$ & $12.8_{\pm 4.6}$ & $88.5_{\pm 0.1}$\\ 
% %   ERM$^{*\diamond}$ & $\times$ & 1x & $74.9_{\pm 2.4}$ & $98.1_{\pm 0.1}$ & $74.9_{\pm 1.7}$ & $98.1_{\pm 0.1}$ & $10.3_{\pm 2.1}$ & $89.3_{\pm 0.2}$ \\ 
% %  ERM$^*$ & $\times$ & 1x & - & - & $80.1_{\pm0.7}$ & $97.8_{\pm 0.3}$ & $23.5_{\pm 5.0}$ & $82.2_{\pm 6.4}$ \\ 
% %  CB$^*$ & $\times$ & 1x & - & - & $71.7_{\pm 1.6}$ & $97.1_{\pm 0.1}$ & $28.4_{\pm 4.7}$ & $77.4_{\pm 7.8}$\\
% %  EIIL &  $\times$ & 1x & $78.7$ & $96.9$ & $83.5_{\pm 2.8}$ & $94.2_{\pm 1.3}$ & $45.5_{\pm 3.2}$ & $51.1_{\pm 3.2}$\\
% %  % LfF &  $\times$ &  2x & & & & \\
% %  JTT &  $\times$ & 5x-6x & $86.7$ & $93.3$ & $83.1_{\pm 3.5}$ & $90.6_{\pm 0.3}$ & $15.7_{\pm 1.6}$ & $85.7_{\pm 0.4}$\\
% %  % CnC & $\times$ & 2x-12x & & & & \\
% %  \SPARE & $\times$ & 1x & ${89.8}_{\pm 0.6}$ & $94.2_{\pm1.6}$ & $91.6_{\pm 0.8}$ & $96.2_{\pm 0.6}$ & $50.6_{\pm 1.3}$ & $59.5_{\pm 4.9}$\\
% %  \midrule\midrule
% %  SSA &  validation & 1.5x-5x &  $89.0_{\pm 0.6}$ & $92.2_{\pm 0.9}$ & $85.1_{\pm 1.3}$ & $96.7_{\pm 1.6}$ & $47.8_{\pm 1.7}$ & $62.1_{\pm 8.2}$ \\ 
% %  % $\text{DFR}^{Tr}_{Tr}$ &  training sub. & $\approx$ 1x &  $90.2_{\pm 0.8}$ & $97.0_{\pm 0.3}$ & $90.27_{\pm 2.14}$ & $97.02_{\pm 0.46}$ & $48.01_{\pm 9.21}$ & $63.77_{\pm 12.89}$  \\
% %  $\text{DFR}^{Val}_{Tr}$ & validation & 1x & $92.9_{\pm 0.2}$ & $94.2_{\pm 0.4}$  & $90.6_{\pm 0.4}$ & $93.4_{\pm 0.2}$ & $50.8_{\pm 1.8}$ & $63.8_{\pm 1.1}$ \\
% %  % DISPEL & training sub. & $\approx$ 1x &  $90.2_{\pm 0.7}$ & $94.3_{\pm 0.2}$ & $90.36_{\pm 0.39}$ & $97.00_{\pm 0.23}$  & $33.80_{\pm 2.24}$ & $79.07_{\pm 1.31}$ \\
% %  \DISPEL  & validation & 1x & $92.8_{\pm 0.6}$  & $94.2_{\pm0.2}$  & $92.7_{\pm 0.4}$ & $94.4_{\pm 0.6}$ & $51.9_{\pm 1.2}$ & $65.2_{\pm 1.6}$ \\ \midrule\midrule
% %  GB & training & 1x &   - & - & $88.1_{\pm 0.6}$ & $95.5_{\pm 0.4}$ & $50.6_{\pm 1.1}$ & $64.3_{\pm 2.1}$ \\
% %  GB$^*$ & training & 1x & -  & - & $87.5_{\pm 0.9}$ & $93.4_{\pm 2.5}$ & $50.8_{\pm 1.9}$ & $61.7_{\pm 7.7}$ \\
% %  GDRO &  training & 1x &  $86.0$ & $93.2$ & $85.7_{\pm 0.8}$ & $94.3_{\pm 1.0}$ & $50.7_{\pm 0.7}$ & $65.1_{\pm 1.2}$\\
% % \bottomrule
% % \end{tabular}%
% % }
% % \end{center}
% % \vspace{-6mm}
% % \end{table*}

%  In the spurious correlation literature, it has become standard to initialize models using weights from publicly available pretrained models. In particular in vision tasks, the ImageNet pretrained weights are commonly used. Here, we explore different pre-trained weights and evaluate the worst-group accuracy they can achieve using various methods. 

% \textbf{Pre-Training is Essential for Robustness to Spurious Correlations}
% %, while in language tasks, weights such as xxx are often utilized [cite]. 
% We conducted experiments on Waterbirds to compare training from ImageNet pretrained weights with random initialization. The results, shown in Table \ref{tab:pretrain_crucial}, confirm that using pretrained weights is crucial for achieving high worst-group accuracy, which holds true across all methods. \ba{move random init to appendix}

% \textbf{Surprisingly, Fine-Tuning CLIP is Not Robust} CLIP has been shown to demonstrate superior robustness to distribution shift when used with zero-shot inference \cite{radford2021learning, mmcl}. Thus, we investigated whether replacing ImageNet pretrained weights with CLIP-pretrained weights could further improve worst-group accuracy. Surprisingly, as shown in Figure \ref{fig:pretrain}, the answer is no, across both datasets and methods. In fact, CLIP weights even lead to much worse worst-group accuracy, prompting caution when using CLIP pre-trained weights when optimizing for worst-group accuracy due to SC. \sj{expanation for why clip doesn't work in 1 line?} \ba{let's see if we can find another network, we cannot say CLIP is not good but we use it!}

%Our hypothesis is that since the CLIP pretrained model has learned more diverse features, potentially including both core and spurious features, it does not benefit the learning of core features but rather makes the learning noisier compared to ImageNet pretrained weights, which are likely more focused on main object features. Another point to note is that while the CLIP paper demonstrates that zero-shot inference with CLIP can outperform ImageNet in out-of-distribution (OOD) generalization, recent work \citep{mmcl} suggests that this is largely due to the zero-shot inference, and finetuning can degrade robustness. For future research, we believe that further investigating this phenomenon to seek explanations, or exploring if special treatment is needed when using CLIP-pretrained weights to improve performance, are valuable directions.

% \textbf{Smaller Models are Equally Robust to SC} Finally, we explore the effect of model size by comparing ResNet18 and ResNet50. As shown in Figure \ref{fig:pretrain}, ResNet18 can achieve robustness on par with ResNet50, and even outperforms ResNet50 on SpuCoSun. This could be because, given that SpuCoSun is the most challenging task, a smaller model size might help to limit overfitting to spurious labels in this scenario. 
% \ba{compare the group inference using different pretrained models. This's interesting and you can use majority in minority metric for it.}

%\sj{can we expand this more? think about other even smaller architectures? or R18 trained with some other training mechanism? small is criticla so we can quickly run the experiments needed}

% \begin{itemize}
%     \item CLIP R50 is worse than ImageNetR50. This is perhaps surprising since the CLIP paper shows that with zero-shot inference CLIP can do better in OOD generalization than ImageNet. However, recent work \citep{mmcl} shows that this is attributed in large part to the zero-shot inference which aligns with our findings that using CLIP with finetuning 
%     \item SWAG if does better, consider why?
% \end{itemize}



==> problem_formulation.tex <==
\section{Background}


\subsection{Problem Formulation}
Let $\mathcal{D}=\{(\x_i,y_i)\}_{i=1}^n$ be the training data with input features $\x_i \in \mathbb{R}^d$ and labels $y_i \in [\mathcal{C}]$ where $\mathcal{C} = \{C_1, ..., C_l\}$ are the classes in dataset $\mathcal{D}$.
%
Machine learning models are trained by minimizing an empirical risk function (ERM) using (stochastic) gradient descent. The goal of ERM is to minimize the average error on the entire training data $\mathcal{D}$: 
\begin{align}\label{eq:erm}
    %\LL_\D(\w)=
    \w^*\in \argmin_{\w}
    \E_{(\x_i,y_i)\in\D}[l(f(\w,\x_i),y_i)],
\end{align}
where $\w$ is the model parameter, and $f(\w,\x_i)$ and $l(f(\w,\x_i),y_i)$ are the output of the network and the loss associated with a training example $(\x_i, y_i)$, respectively.

\textbf{Core and Spurious Features} %Let the dataset $\mathcal{D}$ be partitioned into $\mathcal{C} = \{C_1, ..., C_m \}$ classes. 
Each class is represented by a unique \textit{core} feature. Let $\mathcal{F}$ be the set of \textit{core} features where $f_j\in \mathcal{F}$ is the \textit{core} feature for class $C_j$. The \textit{core} feature is indicative of class membership and as such, is present at both \textit{training} and \textit{test} time. Additionally, let $\mathcal{S}$ be a set of \textit{spurious} features that can be shared between classes. These features are present in the data at \textit{training} time, but are not indicative of class membership and hence, may or may not appear at \textit{test} time.

For example, in the Waterbirds dataset \cite{sagawa2020distributionally}, where the task is to distinguish between \textit{waterbirds} and \textit{landbirds}, the \textit{core} features are the physical characteristics of the birds (e.g. shape of beak, wings) and the \textit{spurious} features are the backgrounds (e.g. ocean, river, lake, tree, grass).

\textbf{Groups}
Examples in the dataset can be partitioned into different groups $g_{f_j, s_k}$, based on the combinations of their core and spurious features $(f_j, s_k)$. If at training time, the majority of examples in class $C_j$ belong to the group $(f_j, s_k)$ i.e. the majority group and $s_k$ doesn't appear frequently in examples of other classes, we say $s_k$ is spurious correlated with class $C_j$. If the model now relies on the spurious feature $s_k$ at training time to classify the majority group of examples in class $C_j$, this will result in a poor accuracy at \textit{test} time on \textit{minority} groups of class $C_j$ i.e. groups that do not contain the spurious feature $s_k$ . This is captured by the worst-group error:

\textbf{Worst-group error} We quantify the performance of the model based on its highest test error across groups $\mathcal{G}=\{\cup_{f_j,s_k}~g_{f_j, s_k}\}$ in all classes. Formally, \textit{worst-group} test error is defined as:
\begin{equation}
    \text{Err}_{wg}=\max_{g\in \mathcal{G}}\E_{(\x_i,y_i)\in g}\!\![
    y_i\neq \hat{y}(\w,\x_i)
    % l_{0,1}(\w,(\x,y))
    ],
\end{equation}
% where $l_{0,1}$ is the 0-1 loss. 
where $\hat{y}(\w,\x_i)$ is the label predicted by the model.
In other words, $\text{Err}_{wg}$ measures the highest fraction of examples that are incorrectly classified across all groups. 

For example, in the Waterbirds dataset, it is possible that due to the correlation between \textit{water} backgrounds and \textit{waterbirds}, the model learns to classify \textit{waterbirds} using the spurious feature i.e the background rather than the core feature i.e. the characteristics of the birds at \textit{training} time. However, the \textit{water} background does not actually determine if a given bird is a \textit{waterbird} and as such will result in extremely high worst-group error on \textit{waterbirds} found on \textit{land} backgrounds. %at \textit{test} time. 

%$, \textit{attribute imbalance} and \textit{attribute (domain) generalization} \cite{yang2023change}. 

\textbf{Validation Set}
Algorithms to improve poor test time worst-group accuracy due to spurious correlations rely on a model selection criteria (hyper-parameter tuning criteria) determined using a validation set where the group membership of examples is known. Formally,

\begin{equation}
    h_* = \argmax_{h} \bigg[ \text{Err}^{V}_{wg} (\mathcal{A}(h, D)) \bigg]
\end{equation}
where $\mathcal{A}(h, D)$ is the model trained on dataset $D$ with hyperparameters $h$ for algorithm $\mathcal{A}$ and $V$ is the group-labeled validation set. 

\textbf{Disambiguation from Other Forms of Distribution Shift}
Other commonly studied distribution shifts are \textit{class imbalance}: different classes are represented unequally in the training set; \textit{feature (attribute) imbalance}: different features (attribute) represented unequally in training set, without any class bias, leading to less confident predictions for underrepresented attributes; \textit{domain (attribute) generalization}: examples from certain domains (attributes) seen at test time do not appear in the training set \cite{yang2023change}.  
The problem of poor worst-group accuracy due to spurious correlations differs in its cause: spurious feature (attribute) appears correlated with a class in training set but not at test time and its effect: predictions biased towards spuriously correlated class at test time when the spurious feature (attribute) appears. 

\subsection{Methods}

\begin{table}[h]
    \centering
    \begin{tabular}{l|c|}
     Method&Type (GI / RT)\\   \hline
 ERM& RT\\
 JTT& GI\\
 EIIL& GI\\
 SPARE& GI\\
 SSA&GI + RT\\
 DFR&RT\\
 LRMIX&RT\\
 GB&RT\\
 GDRO&RT\\
 PDD&RT\\\end{tabular}
    \caption{Categorization of Existing Methods (GI = Group Inference, RT = Robust Training)}
    \label{tab:categorization_of_methods}
\end{table}


Existing methods to tackle worst-group accuracy due to spurious correlations can be broadly characterized into two phases: group inference, where group membership is inferred on the training set, and robust training where this group information is used to train a model that doesn't suffer from poor worst-group accuracy.

\textbf{Model Selection Criterion}
All methods rely on a group-labeled validation set to tune the hyperparameters in both the group inference and robust training phase. We refer to this as the model selection criterion. 

\subsection{Datasets}

% \textbf{SpuCoMNIST}
% \ba{I'm not sure if we should include this in details in the main paper. People wont be excited about it and it's not a realistic dataset to benchmark (this time our focus is benchmarking not studying a particular parameter). This can be a side discussion with details in appendix.}

\textbf{SpuCoAnimals} a large scale vision dataset curated from ImageNet with \textit{two} realistic spurious correlations \cite{russakovsky2015imagenet}. \animals\ has 4 classes: \textit{landbirds}, \textit{waterbirds}, \textit{small dog} breeds and \textit{big dog} breeds\footnote{\textit{Small} dog refers to \textit{toy} or \textit{toy terrier} breeds, often kept as companion pets and \textit{big} dog breeds refer to both medium-sized and large-sized breeds, known for their working abilities, guarding skills or specific purposes. Exact ImageNet classes corresponding to each \animals' class can be found in Appendix \ref{appendix:spuco_animals}}. Waterbirds and Landbirds are spuriously correlated with \textit{water} and, \textit{land} backgrounds, respectively. Small dogs and big dogs are spuriously correlated with \textit{indoor} and \textit{outdoor} backgrounds, respectively. The training set has 10500 examples per class with a 20:1 ratio between majority and minority group for each class. The validation set has 525 examples for each class with the same ratio of majority to minority groups. The test set is group-balanced and has 500 examples per group. 

\textbf{SpuCoSUN} is a dataset featuring four meticulously curated classes designed to emulate real-world environments and objects, ensuring a realistic and practical dataset. Each class seamlessly blends specific background settings from SUN397 with corresponding spurious features from OpenImages V7. The classes include: Recreational and Sports Environments, encompassing amusement parks, athletic fields, and indoor badminton courts, with associated spurious features such as sports equipment; Residential and Living Spaces, focusing on areas like attics, bathrooms, bedrooms, and dining rooms, paired with spurious features like various fruits and vegetables; Cultural and Educational Institutions, comprising locations like abbeys, amphitheaters, art galleries, and libraries, with associated spurious features like different types of baked goods; and Transportation and Infrastructure, covering settings like airplane cabins, airport terminals, bridges, and train stations, paired with spurious features related to containers and storage. Each class exhibits one majority group (own spurious) and three minority groups (spurious of other three classes), maintaining a ratio of 67:1 in the training and validation set and 1:1 in the test set. The training set comprises approximately 32,000 images, the validation set is about 25\% of the training set's size, and the test set consists of 250 images per group.

Additional details about the dataset construction appear in Appendix \ref{app:dataset_construction}. 
% SpuCoSun features four carefully curated classes, designed to reflect real-world environments and objects, ensuring the dataset’s realism and practicality. Each class combines specific background settings from SUN397 with corresponding spurious features from OpenImages V7. The classes are as follows:

% \begin{itemize}[label=--, left=0em, itemsep=0.5em]
%     \item \textbf{Recreational and Sports Environments:}
%     \begin{itemize}[label=$\circ$, left=1em, itemsep=0.5em]
%         \item Includes amusement parks, athletic fields, and indoor badminton courts.
%         \item Associated spurious features: sports equipment such as volleyballs, footballs, golf balls, and tennis balls.
%     \end{itemize}

%     \item \textbf{Residential and Living Spaces:}
%     \begin{itemize}[label=$\circ$, left=1em, itemsep=0.5em]
%         \item Focuses on residential and personal living spaces like attics, bathrooms, bedrooms, and dining rooms.
%         \item Associated spurious features: various fruits and vegetables like pumpkins, watermelons, tomatoes, broccoli, and bell peppers.
%     \end{itemize}

%     \item \textbf{Cultural and Educational Institutions:}
%     \begin{itemize}[label=$\circ$, left=1em, itemsep=0.5em]
%         \item Comprises locations like abbeys, amphitheaters, art galleries, and libraries.
%         \item Associated spurious features: different types of baked goods such as bread, cookies, muffins, bagels, and pretzels.
%     \end{itemize}

%     \item \textbf{Transportation and Infrastructure:}
%     \begin{itemize}[label=$\circ$, left=1em, itemsep=0.5em]
%         \item Covers transportation and infrastructure settings like airplane cabins, airport terminals, bridges, and train stations.
%         \item Associated spurious features: items related to containers and storage such as flowerpots, waste containers, bottles, beakers, and barrels.
%     \end{itemize}
% \end{itemize}

% Each class has 1 majority group (own spurious) and 3 minority groups (spurious of other 3 classes). The ratio of majority to minority is 67:1 in the training and validation set and 1:1 in the test set. The training set is approximately 32k images, the validation set is approximately 25\% of the size of the training set, and the test set consists of 250 images per group.
